Usable Privacy in Virtual Worlds: Design Implications for Data Collection Awareness and Control Interfaces in Virtual Reality

Extended reality (XR) devices have become ubiquitous. They are equipped with arrays of sensors, collecting extensive user and environmental data, allowing inferences about sensitive user information users may not realize they are sharing. Current VR privacy notices largely replicate mechanisms from 2D interfaces, failing to leverage the unique affordances of virtual 3D environments. To address this, we conducted brainstorming and sketching sessions with novice game developers and designers, followed by privacy expert evaluations, to explore and refine privacy interfaces tailored for VR. Key challenges include balancing user engagement with privacy awareness, managing complex privacy information with user comprehension, and maintaining compliance and trust. We identify design implications such as thoughtful gamification, explicit and purpose-tied consent mechanisms, and granular, modifiable privacy control options. Our findings provide actionable guidance to researchers and practitioners for developing privacy-aware and user-friendly VR experiences.

==> temp.tex <==
\subsubsection{Challenges}
Within the challenges, we grouped five themes: \emph{Problems, risks, responsibility, trade-off,} and \emph{questions}, which we used to cover the different aspects mentioned during the focus group that addressed challenges and things to consider when creating privacy mechanisms for XR environments.
\begin{description}
    %6
    \item[Problems] Overall, the experts identified two main areas of problems: Those related to the user and those related to the developers and designers.
    
    On the user's side, things such as the users not wanting to deal with privacy notices were mentioned (E2). In combination with not being able to progress within the game or application without making a privacy choice, this can lead to the users not paying attention to privacy notices and just rushing through them, as mentioned by E4: "I do not think that you make people really carefully read the permissions". The reasons for this, highlighted by the experts, might be that the users are used to encountering an unmanageable number of privacy choices in current privacy notices (E1, E3). As the different sensors in XR environments access different types of data, which need to be covered by a privacy mechanism, a solution has to be found to not transfer the same problem into the privacy mechanisms for immersive environments ("I do not want another Cookie Banner" (E1)).
    
    Additionally, even if there are privacy mechanisms implemented, users might still not trust the software to preserve their privacy in the way that it claims to do: "I would only trust the OS to allow then certain sensors to be accessed by the game" (E1).
    
    Regarding the developers, the experts mentioned that a high burden is placed on them (E1). On one hand, they have to consider the requirements of the user, on the other hand, they have to fulfill company requirements (E3). This can mean finding a solution that does not break the immersion while also not spoiling the game too much during the privacy choice (which was considered a risk if the privacy mechanism was tied in too closely to the game mechanics of the corresponding room within the VR escape room ("have something similar, but not in the context of the game, not to spoil it" (E4)).
    
    While thinking about possible improvements or alternative designs, the experts also mentioned they found it "hard to tell how [the mechanism] would actually look in-game" (E2), making the design process harder. This also applies to the design of the alternative game elements, which would need individual solutions depending on the game mechanics (E3) and missing sensor data that has to be replaced somehow.

    \item[Risks] The experts mentioned different risks that could be encountered when dealing with privacy mechanisms in XR environments. While things such as manipulation of the user by "hav[ing] hidden information in the text, like fine print" (E3) or purposefully designing mechanisms in a non-understandable way ("symbols can be designed on purpose in a non-obvious or non-understandable way" (E3)) can occur independently of the context, some are inherent to XR applications: Due to their immersive nature, a privacy mechanism included seamlessly might make it difficult for users to make the distinction between XR and real-world effects of the data collection ("In particular in an immersive game it might not be clear if this is in-game or out of game" (E2)). Expert E2 also argued that to avoid this, it might even be necessary to "break the fourth wall" and thus the immersion. This goes together with the experts' concern that too much gamification could cause users not to take the privacy decision seriously ("Weakness [of this design]: Maybe too much gamification" (E1)).
    
    The experts further mentioned that the alternative game elements that were designed "might still reveal other data" (E2) about the user, which would have to be covered by the privacy mechanism. They also raised concerns about how the designed privacy mechanisms would adapt to a multiplayer scenario (E4).
    
    \item[Responsibility] One reoccurring conflict was the question of responsibility. Due to the multiple parties involved, the experts discussed that it could be either on the side of the application developers or device manufacturers (which would mean that the OS should be the trusted party that handles the privacy mechanism: "I would only want, certain privacy and sensor level based decisions to be asked once by the OS" (E1)). A third option that was brought up was that of legal requirements (E1), which ideally would cover the necessary aspects (but would still leave the implementation with one of the other parties).

    \item[Trade-off] As not all of the previously mentioned aspects go together, some trade-offs were identified by the experts that have to be made when deciding on a specific design for the privacy mechanism. Regarding content, there is a trade-off between complexity and precision versus comprehension and understandability: "This is the big question: How can I have a nice trade-off between complexity and comprehension for the user?" (E3). Depending on how this trade-off is made, it might also interfere with how easy or hard it is to implement ("If you want to make it granular for sensors, it's the easiest to implement, but the hardest to understand" (E2)), as well as the question at what point the user is overwhelmed or even frightened by the information provided which "is kind of in contrast to the transparency company should give" (E3).
    
    Trade-offs regarding the design are whether there should be global settings to not overwhelm the user with too many decisions ("once you have seen the mechanic, you can decide [you] don't want to make this decision again" (E2)), or rather local settings to allow for granular privacy choices which are closely positioned to the corresponding game elements ("I would try to keep it local to the very thing you are currently interacting with." (E2)), as well as the balance between creating a fun, engaging mechanic while still keeping it serious enough so that the purpose of the interaction as a privacy mechanism does not get lost (E1).

    Lastly, related to whose interests are represented, how design decisions are made depends on the trade-off between user and company interests, which can but do not have to align: "I guess a lot of recommendations are quite obvious, but we also know that they will not happen. And that is because of the differences between what company wants and what user wants" (E3).
    
    \item[Questions] The experts raised some questions related to the aforementioned points: When it comes to making privacy decisions, do users "understand what they are doing and what they are selecting" (E1)? To support them, "how would you re-educate users" (E4)  to read and meaningfully interact with privacy policies? And finally, what happens if the user does not make a choice? ("[For design two,] what happens if I do not put it in the tube at all?" (E3)) What does the default look like?
\end{description}
